Is ChatGPT Good at Search? Investigating Large Language Models as Re-Ranking Agents

Large Language Models (LLMs) have demonstrated remarkable zero-shot generalization across various language-related tasks, including search engines. However, existing work utilizes the generative ability of LLMs for Information Retrieval (IR) rather than direct passage ranking. The discrepancy between the pre-training objectives of LLMs and the ranking objective poses another challenge. In this paper, we first investigate generative LLMs such as ChatGPT and GPT-4 for relevance ranking in IR. Surprisingly, our experiments reveal that properly instructed LLMs can deliver competitive, even superior results to state-of-the-art supervised methods on popular IR benchmarks. Furthermore, to address concerns about data contamination of LLMs, we collect a new test set called NovelEval, based on the latest knowledge and aiming to verify the model's ability to rank unknown knowledge. Finally, to improve efficiency in real-world applications, we delve into the potential for distilling the ranking capabilities of ChatGPT into small specialized models using a permutation distillation scheme. Our evaluation results turn out that a distilled 440M model outperforms a 3B supervised model on the BEIR benchmark. The code to reproduce our results is available at www.github.com/sunnweiwei/RankGPT.

==> tables/beir-lite.tex <==
\begin{table*}[!t]
\centering
\small
\setlength\tabcolsep{5pt}
\caption{\textbf{Results (nDCG@10) on BEIR.} Best performing unsupervised and overall system(s) are marked bold.}
\label{table:beir}

\begin{tabular}{l cccccccccc|c }

\toprule
\textbf{Method} & Covid &  NFCorpus &  Touche &  DBPedia & SciFact &  Signal & News &  Robust04 & Avg \\

\midrule

BM25
& 59.47 & 30.75 & \textbf{44.22} & 31.80 & 67.89 & 33.05 & 39.52 & 40.70 & 43.42
\\

\midrule
\textbf{Supervised} \\
\midrule

monoBERT (340M)
& 70.01 & 36.88 & 31.75 & 41.87 & 71.36 & 31.44 & 44.62 & 49.35 & 47.16
\\

monoT5 (220M)
& 78.34 & 37.38 & 30.82 & 42.42 & 73.40 & 31.67 & 46.83 & 51.72 & 49.07
\\

monoT5 (3B)
& 80.71 & \textbf{38.97} & 32.41 & 44.45 &  \textbf{76.57} & 32.55 & 48.49 & 56.71 & 51.36
\\

TART-Rerank (FLAN-T5-XL)
& 75.10 & 36.03 & 27.46 & 42.53 & 74.84 & 25.84 & 40.01 & 50.75 & 46.57
\\

Cohere Rerank-v2
& 81.81 & 36.36 & 32.51 & 42.51 & 74.44 & 29.60 & 47.59 & 50.78 & 49.45
\\


Cohere Embedding-large
& 80.1 & 34.7 & 27.6 & 37.2 & 72.1 & 30.6 & 46.1 & 48.9 & 47.2
\\

OpenAI Embedding-ada
& 81.3 & 35.8 & 28.0 & 40.2 & 73.6 & 32.9 & 49.5 & 50.9 & 49.0
\\


% InstructOR (335M)$^\dagger$
% & 56.1 & 33.0 & 25.5 &  38.2 & 60.9
% \\

% InstructOR (1.5B)$^\dagger$
% & 53.7 & 33.0 & 21.0 & 37.7 & 62.7
% \\


\midrule
\textbf{Unsupervised} \\
\midrule

UPR (FLAN-T5-XL)
& 68.11 & 35.04 & 19.69 & 30.91 & 72.69 & 31.91 & 43.11 & 42.43 & 42.99
\\

% SGPT-CE (6.1B)
% & 79.1 & 34.7 & 23.4 & 37.0 & 68.2 & 32.3 & 46.6 & 48.0 & 46.16
% \\

InPars (monoT5-3B)$^\dagger$
& 78.35 & - & - & - & - & - & - & - & -
\\

% HyDE (\code{text-davinci-003})
% & 59.3 & - & 27.3 & - & 44.0 & - & 46.6 & - & 36.8 & 69.1
% \\

Promptagator++ (zero-shot)$^\dagger$
& 76.0 & 36.0 & 27.8 & 41.3 & 73.6 & - & - & - & -
\\

Promptagator++ (few-shot)$^\dagger$
& 76.2 & 37.0 & 38.1 & 43.4 & 73.1 & - & - & - & -
\\


\midrule
\multicolumn{5}{l}{LLM API (Permutation generation)}\\
\midrule

\code{gpt-3.5-turbo}
& 76.67 & 35.62 & 36.18 & 44.47 & 70.43 & 32.12 & 48.85 & 50.62 & 49.37
\\

\quad + \code{gpt-4} Rerank$^\ddagger$
& \textbf{85.51} & \textbf{38.47} & \textbf{38.57} & \textbf{47.12} & \textbf{74.95} & \textbf{34.40} & \textbf{52.89} & \textbf{57.55} & \textbf{53.68}
\\

\bottomrule
\end{tabular}

\begin{tablenotes}
  \small
  
  \item $^\dagger$ InPars re-ranks the top-1000 BM25 passages, while Promptagator++ re-ranks the top-200 Promptagator retrieved passages. The results for these two models are cited from original papers. All other models re-rank the same BM25 top-100 passages.
  
  \item $^\ddagger$ We use \code{gpt-4} to re-rank the top-30 passages re-ranked by \code{gpt-3.5-turbo} to reduce the cost of calling \code{gpt-4} API.
  
\end{tablenotes}

\end{table*}


==> tables/beir.tex <==
\begin{table*}[!t]
\centering
\setlength\tabcolsep{5pt}
\caption{Results (nDCG@10) on BEIR. }
\label{table:beir}

\begin{tabular}{l cccccccccc c }

\toprule
\textbf{Method} & Covid &  NFCorpus & FiQA &  Signal & News &  Robust04 & ArguAna &  Touche &  DBPedia & SciFact & Avg \\

\midrule

BM25
& 59.47 & 30.75 & 23.61 & 33.05 & 39.52 & 40.70 & 29.99 & 44.22 & 31.80 & 67.89 & 43.42
\\

\midrule
\textbf{Supervised} \\
\midrule

monoBERT (340M)
& 70.01 & 36.88 & 36.23 & 31.44 & 44.62 & 49.35 & 38.58 & 31.75 & 41.87 & 71.36 & 47.16
\\

monoT5 (220M)
& 78.34 & 37.38 & 39.22 & 31.67 & 46.83 & 51.72 & 23.19 & 30.82 & 42.42 & 73.40 & 49.07
\\

monoT5 (3B)
& 80.71 & 38.97 & 45.77 & 32.55 & 48.49 & 56.71 & 35.43 & 32.41 & 44.45 &  76.57 & 51.36
\\

TART-Rerank (FLAN-T5-XL)
& 75.10 & 36.03 & 37.42 & 25.84 & 40.01 & 50.75 & 39.11 & 27.46 & 42.53 & 74.84 & 46.57
\\

InstructOR (335M)$^\dagger$
& 56.1 & 33.0 & 44.6 & - & - & - & 51.5 & 25.5 &  38.2 & 60.9
\\

InstructOR (1.5B)$^\dagger$
& 53.7 & 33.0 & 47.6 & - & - & - & 51.8 & 21.0 & 37.7 & 62.7
\\


\midrule
\textbf{Unsupervised} \\
\midrule

UPR (FLAN-T5-XL)
& 68.11 & 35.04 & 34.58 & 31.91 & 43.11 & 42.43 & 29.63 & 19.69 & 30.91 & 72.69 & 42.99
\\

InPars (monoT5-3B)$^\dagger$
& 78.35 & - & - & - & - & - & - & - & - & -
\\

% HyDE (\code{text-davinci-003})
% & 59.3 & - & 27.3 & - & 44.0 & - & 46.6 & - & 36.8 & 69.1
% \\

Promptagator++ (zero-shot)$^\dagger$
& 76.0 & 36.0 & 45.9 & - & - & - & 53.1 & 27.8 & 41.3 & 73.6
\\


\midrule
\multicolumn{5}{l}{LLM API (Sliding Listwise)}\\
\midrule

\code{gpt-3.5-turbo}
& 76.67 & 35.62 & 31.57 & 32.12 & 48.85 & 50.62 & & 36.18 & 44.47 & 70.43
\\

\quad + \code{gpt-4} Rerank$^\ddagger$
& 85.51 & & & 34.40 & 52.89 & 57.55 & &38.57 && 74.95
\\


\midrule

\code{gpt-3.5-turbo} \emph{+Instruction}
& 75.64
\\

\quad + \code{gpt-4} Rerank \emph{+Instruction}$^\ddagger$
\\

\bottomrule
\end{tabular}

\begin{tablenotes}
  \small
  
  \item $^\dagger$ InstructOR is a text embedding model that directly retrieves passage from corpus. InPars re-rank top-1000 BM25 passages. Promptagator++ re-rank top-200 passages retrieved by Promptagator dense retrieval model. Since these 3 methods do not have open-source code, we directly cite the results from original papers. For all other models, we use the same BM25 top-100 passages for a fair comparison.
  
  \item $^\ddagger$ We use \code{gpt-4} to re-rank the top-30 passages re-ranked by \code{gpt-3.5-turbo} to reduce the cost of calling \code{gpt-4} API.
  
\end{tablenotes}

\end{table*}


==> tables/distillation.tex <==
\begin{table}[!t]
\centering
\small
\setlength\tabcolsep{4pt}
\caption{\textbf{Results (nDCG@10) of specialized models.} Best performing specialized model(s) are marked bold. The label column denotes the relevance judgements used in model training, where MARCO denotes use MS MARCO annotation, ChatGPT denotes use the outputs of permutation generation instructed ChatGPT as labels. BEIR (Avg) denotes average nDCG on eight BEIR datasets, and the detailed results are at Table~\ref{table:distill-beir}.}
\label{table:distill}

\begin{tabular}{c l ccc }

\toprule

Label & Method / Loss & DL19 & DL20 & BEIR (Avg)
\\
\midrule

$\varnothing$ & BM25
& 50.58 & 47.96 & 43.42
\\

$\varnothing$ & ChatGPT
& 65.80 & 62.91 & 49.37
\\

MARCO & monoT5 (3B)
& 71.83 & 68.89 & 51.36
\\

\midrule

MARCO & Pointwise BCE
& 65.57 & 56.72 & 39.43
\\

MARCO & Listwise CE
& 65.99 & 57.97 & 35.45
\\


MARCO & RankNet
& 66.34 & 58.51 & 38.79
\\

MARCO & LambdaLoss
& 64.82 & 56.16 & 40.62
\\

\midrule

ChatGPT & Listwise CE
& 65.39 & 58.80 & 47.74
\\

ChatGPT & RankNet
& 66.56 & 59.43 & \textbf{50.53}
\\

ChatGPT & LambdaLoss
& \textbf{67.17} & \textbf{60.56} & 49.77
\\

\bottomrule
\end{tabular}
\end{table}


==> tables/dl19-prompt.tex <==
\begin{table}[!t]
\centering
\setlength\tabcolsep{5pt}
\caption{Results on TREC-DL19. All models re-rank the top-100 passages retrieved by BM25.}
\label{table:dl19}

\begin{tabular}{l ccc }

\toprule
\textbf{Method} & nDCG@1 & nDCG@5 & nDCG@10 \\

\midrule

BM25
& 54.26 & 52.78 & 50.58 
\\

\midrule
\textbf{Supervised} \\
\midrule

monoBERT (340M)
& 79.07 & 73.25 & 70.50
\\

monoT5 (220M)
& 79.84 & 73.77 & 71.48
\\

monoT5 (3B)
& 79.07 & 73.74 & 71.83
\\

\midrule
\textbf{Unsupervised} \\
\midrule

UPR (3B)
\\

InPars (3B)
\\

\midrule
\textbf{LLM} \\
\midrule

text-curie-001 \emph{yes-no}$^\dagger$
& \\

text-davinci-003 \emph{yes-no}$^\dagger$
& \\



\midrule

text-curie-001 \emph{qgp}
& 50.78 & 50.77 & 49.76 \\

text-davinci-003 \emph{qgp}
& \\


\midrule

text-curie-001 \emph{listwise}
& \\

text-davinci-003 \emph{listwise}
& \\

gpt-3.5-turbo \emph{listwise}
& 82.17 & 71.15 & 65.80
\\

gpt-4 \emph{listwise}
& \textbf{82.56} & \textbf{79.16} & \textbf{75.59}
% & 76.74 & 69.79 & 66.91
% & 81.01 & 69.65 & 64.62
\\

\bottomrule
\end{tabular}
\begin{tablenotes}
  \small
  \item $^\dagger$ Yes-no prompting uses 4 in-context examples, following HELM.
\end{tablenotes}
\end{table}


==> tables/dl20.tex <==
\begin{table}[!t]
\centering
\setlength\tabcolsep{5pt}
\caption{Results on TREC-DL20. All models re-rank the top-100 passages retrieved by BM25.}
\label{table:dl20}

\begin{tabular}{l ccc }

\toprule
\textbf{Method} & nDCG@1 & nDCG@5 & nDCG@10 \\

\midrule

BM25
& 57.72 & 50.67 & 47.96
\\

\midrule
\textbf{Supervised} \\
\midrule

monoBERT (340M)
& 78.70 & 70.74 & 67.28
\\

monoT5 (220M)
& 77.47 & 69.40 & 66.99
\\

monoT5 (3B)
\\

\midrule
\textbf{Unsupervised} \\
\midrule

UPR (3B)
\\

InPars (3B)
\\

\midrule
\textbf{LLM} \\
\midrule

text-curie-001 \emph{yes-no}$^\dagger$
& \\

text-davinci-003 \emph{yes-no}$^\dagger$
& \\



\midrule

text-curie-001 \emph{qgp}
\\

text-davinci-003 \emph{qgp}
& \\


\midrule

text-curie-001 \emph{listwise}
& \\

text-davinci-003 \emph{listwise}
& \\

gpt-3.5-turbo \emph{listwise}
\\

gpt-4 \emph{listwise}

\\

\bottomrule
\end{tabular}
\begin{tablenotes}
  \small
  \item $^\dagger$ Yes-no prompting uses 4 in-context examples, following HELM.
\end{tablenotes}
\end{table}


==> tables/trec.tex <==
\begin{table*}[!t]
\centering
\small
\setlength\tabcolsep{2.5pt}
\caption{\textbf{Results on TREC-DL19 and TREC-DL20.} All models (except InPars) re-rank the top-100 passages retrieved by BM25. Best performing unsupervised and overall system(s) are marked bold.}
\label{table:trec}

\begin{tabular}{l l ccc ccc}

\toprule


& & \multicolumn{3}{c}{\textbf{DL19}} 
& \multicolumn{3}{c}{\textbf{DL20}} 
\\

\textbf{Method}  & & nDCG@1 & nDCG@5 & nDCG@10 & nDCG@1 & nDCG@5 & nDCG@10 \\

\midrule

BM25 &
& 54.26 & 52.78 & 50.58 
& 57.72 & 50.67 & 47.96
\\

\midrule
\textbf{Supervised} \\
\midrule

monoBERT (340M) &
& 79.07 & 73.25 & 70.50
& 78.70 & 70.74 & 67.28
\\

monoT5 (220M) &
& 79.84 & 73.77 & 71.48
& 77.47 & 69.40 & 66.99
\\

monoT5 (3B) &
& 79.07 & 73.74 & 71.83
& \textbf{80.25} & 72.32 & 68.89
\\

Cohere Rerank-v2 &
& 77.13 & 76.17 & 73.22
& 79.32 & 71.00 & 67.08
\\

\midrule
\textbf{Unsupervised} \\
\midrule

UPR (FLAN-T5-XL) &
& 51.55 & 53.71 & 53.85
& 63.27 & 59.41 & 56.02
\\

InPars (monoT5-3B)$^\dagger$ &
&- & - & -
& - & - & 66.12
\\

% \multicolumn{2}{l}{HyDE (\code{text-davinci-003})}
% & - & - & 61.3
% & - & - & 57.9
% \\

\midrule
LLM API & Instruction methods\\
\midrule

\code{text-curie-001} & Relevance generation (4-shot)
& 39.53 & 40.02 & 41.53
& 41.98 & 34.80 & 34.91
\\

% \code{text-davinci-003} \quad \emph{yes-no}$^\dagger$
% & \\



% \midrule

\code{text-curie-001} & Query generation
& 50.78 & 50.77 & 49.76 
& 50.00 & 48.36 & 48.73
\\

\code{text-davinci-003} & Query generation
& 37.60 & 44.73 & 45.37
& 51.25 & 47.46 & 45.93
\\


% \midrule


\code{text-davinci-003} & Permutation generation
& 69.77 & 64.73 & 61.50
& 69.75 & 58.76 & 57.05
\\

\code{gpt-3.5-turbo} & Relevance generation (100)
& 69.38 & 64.14 & 61.15
& 70.68 & 60.02 & 57.72

\\

\code{gpt-3.5-turbo} & Permutation generation
& 82.17 & 71.15 & 65.80
& \textbf{79.32} & 66.76 & 62.91
\\

\code{gpt-4} & Permutation generation
& \textbf{82.56} & \textbf{79.16} & \textbf{75.59}
& 78.40 & \textbf{74.11} & \textbf{70.56}
% & 76.74 & 69.79 & 66.91
% & 81.01 & 69.65 & 64.62
\\

\bottomrule
\end{tabular}
\begin{tablenotes}
  \small
  
  \item $^\dagger$ InPars re-rank top-1000 BM25 passages. We cite its results from original paper.
  
\end{tablenotes}

\end{table*}

